Improving Approximation Guarantees for Maximin Share

We consider fair division of a set of indivisible goods among $n$ agents with additive valuations using the fairness notion of maximin share (MMS). MMS is the most popular share-based notion, in which an agent finds an allocation fair to her if she receives goods worth at least her ($1$-out-of-$n$) MMS value. An allocation is called MMS if all agents receive their MMS values. However, since MMS allocations do not always exist, the focus shifted to investigating its ordinal and multiplicative approximations. In the ordinal approximation, the goal is to show the existence of $1$-out-of-$d$ MMS allocations (for the smallest possible $d>n$). A series of works led to the state-of-the-art factor of $d=\lfloor3n/2\rfloor$ [Hosseini et al.'21]. We show that $1$-out-of-$4\lceil n/3\rceil$ MMS allocations always exist, thereby improving the state-of-the-art of ordinal approximation. In the multiplicative approximation, the goal is to show the existence of $\alpha$-MMS allocations (for the largest possible $\alpha < 1$), which guarantees each agent at least $\alpha$ times her MMS value. We introduce a general framework of "approximate MMS with agent priority ranking". An allocation is said to be $T$-MMS, for a non-increasing sequence $T = (\tau_1, \ldots, \tau_n)$ of numbers, if the agent at rank $i$ in the order gets a bundle of value at least $\tau_i$ times her MMS value. This framework captures both ordinal approximation and multiplicative approximation as special cases. We show the existence of $T$-MMS allocations where $\tau_i \ge \max(\frac{3}{4} + \frac{1}{12n}, \frac{2n}{2n+i-1})$ for all $i$. Furthermore, we can get allocations that are $(\frac{3}{4} + \frac{1}{12n})$-MMS ex-post and $(0.8253 + \frac{1}{36n})$-MMS ex-ante. We also prove that our algorithm does not give better than $(0.8631 + \frac{1}{2n})$-MMS ex-ante.

==> acks.tex <==
% In the interest of anonymization, please do not include acknowledgements in your submission.
%\begin{acks}
%
% The authors would like to thank Dr. Maura Turolla of Telecom Italia
% for providing specifications about the application scenario.
%
% The work is supported by the
% \grantsponsor{GS501100001809}{National Natural Science Foundation of China}{http://dx.doi.org/10.13039/501100001809}
% under Grant No. \grantnum[http://www.nnsf.cn/youngscientsts]{GS501100001809}{Young Scientsts' Support Program}.
%
%\end{acks}


==> conclusion.tex <==
\section{Conclusion}
In this work, we study various relaxations of MMS. First we prove the existence of $1$-out-of-$4\ceil{\frac{n}{3}}$ MMS allocations which improves the state-of-the-art $1$-out-of-$\floor{\frac{3n}{2}}$ factor by~\cite{Hosseini2021OrdinalMS}. Since even the non-existence of $1$-out-of-$(n+1)$ MMS allocations is open to this date, one obvious future direction is to reduce the gap between the lower and upper bounds for ordinal MMS by improving either of the bounds.

Furthermore, we introduce a general framework of \emph{approximate MMS with agent priority ranking} which captures both ordinal approximation and multiplicative approximations of MMS as special cases. This framework introduces so many directions since by setting $T \defeq (\tau_1, \ldots, \tau_n)$ for different values of $\tau_1, \ldots, \tau_n$, different MMS guarantees would be addressed. In particular we prove the existence of $T$-MMS allocations where $\tau_i \ge \max(\frac{3}{4} + \frac{1}{12n}, \frac{2n}{2n+i-1})$ for all $i$. 

Finally, by ordering the agents randomly, we can get allocations that are $(\frac{3}{4} + \frac{1}{12n})$-MMS ex-post and $(0.8253 + \frac{1}{36n})$-MMS ex-ante, touching upon the sought-after ``best-of-both-worlds'' guarantees. While improving the ex-post guarantee for MMS is very interesting and challenging on its own, improving ex-ante guatantees while having $\frac{3}{4}$-MMS ex-post is another interesting direction.


==> middle-ground.tex <==
\section{\texorpdfstring{$(\alpha, \beta, \gamma)$}{(alpha, beta, gamma)}-MMS Allocation}\label{sec:or}

In this section, we show the existence of $(2(1-\beta)/\beta, \beta, 3/4)$-MMS allocation for any $3/4 < \beta < 1$. Using $\beta = \sqrt{3}/2$, this implies the existence of a randomized allocation that gives each agent at least $3/4$ times her MMS value (ex-post) and at least $(34\sqrt{3} - 48)/8\sqrt{3} > 0.785$ times her MMS value in expectation (ex-ante). 

Given an instance $\ins$, without loss of generality, we assume that $\I$ is $n$-normalized and ordered, which implies that $\MMS_i = 1,\forall i\in N$. Since our approach is an extension of the Garg-Taki (GT) algorithm~\cite{garg2021improved} for the existence of $3/4$-MMS allocation, we first summarize their algorithm. GT algorithm has two phases of \emph{valid reductions} and \emph{bag filling}. In a valid reduction, the instance is reduced by removing an agent $a$ and a subset $S$ of goods such that $a$'s value for $S$ is at least $3/4$, and the MMS values of the remaining agents do not decrease, i.e., $v_a(S) \ge 3/4$ and $\MMS_i \ge 1$ for each remaining agent in the reduced instance $(N\setminus\{a\}, M\setminus\{S\}, V\setminus\{v_a\})$.

The GT algorithm utilizes the simple valid reductions with the set of goods $S_1= \{1\}$ (i.e., the highest valued good), $S_2 = \{n, n+1\}$, $S_3 = \{2n-1, 2n, 2n+1\}$, and $S_4=\{1, 2n+1\}$, in the priority order of $S_1$, $S_2$, $S_3$, and $S_4$, i.e., $S_k$ is performed only when for all $j<k$, $S_j$ is not feasible. The following lemma (proof is in Appendix~\ref{app}) shows that for all $k\in[4]$, $S_k$ is a valid reduction if performed in the priority order. 

\begin{restatable}{lemma}{validred}\cite{garg2021improved}
Let $S$ be the lowest index bundle in $S\in\{S_1,S_2,S_3,S_4\}$ for which $\{i \in N: v_i(S) \geq 3/4 \}$ is non-empty. Then, removing $S$ and agent $a$ with $v_a(S) \ge 3/4$ is a valid reduction.
\end{restatable}

Let $\I'=([n'], [m'], V')$ be the instance after all the valid reductions are performed, i.e., no more valid reductions are feasible for $\I'$. This gives some information about the values of goods shown in the following corollary. 

\begin{corollary}\label{cor:val}
If no valid reductions are feasible for $\I'=([n'], [m'], V')$, then for any agent $i\in [n']$, $v_i(1) < 3/4$, $v_i(n'+1) < 3/8$, and $v_i(2n'+1) < 1/4$. 
\end{corollary}
\begin{algorithm}[t!]
\caption{The $(2(1-\beta)/\beta, \beta, 3/4)$-MMS Algorithm}\label{algo:or}
    \textbf{Input:} $n$-normalized ordered instance $\ins$, where $\MMS_i = 1, \forall i\in N$, and $\beta\in (3/4, 1)$\\
    \textbf{Output:} $(2(1-\beta)/\beta, \beta, 3/4)$-MMS allocation $A$
\begin{algorithmic}[1]
  \State $N_1 \gets$ an arbitrary set of agents s.t. $|N_1| \le 2(1-\beta)|N|/\beta$, with a target of at least $\beta$-MMS
  \State $N_2 \gets N\setminus N_1$, set of remaining agents ($|N_2| \ge (3\beta -2)|N|/\beta$), with a target of at least $3/4$-MMS
  \State $S_1\gets \{1\}$;\ \ $S_2\gets \{|N|, |N|+1\}$;\ \ $S_3\gets \{2|N|-1, 2|N|, 2|N|+1\}$;\ \ $S_4\gets\{1, 2|N|+1\}$
  \State $T_1 \gets \{i\in N_1: \exists k\in [4], v_i(S_k) \ge \beta\}$; \ \ $T_2 \gets \{i\in N_2: \exists k\in [4], v_i(S_k) \ge 3/4\}$
  \While{$T_1 \cup T_2 \neq \emptyset$} \Comment{Valid Reductions}
	   \State $\ell\gets$ smallest index s.t. either $v_i(S_\ell) \ge \beta$, for some $i\in N_1$ or $v_i(S_\ell) \ge 3/4$, for some $i\in N_2$
	   \State $a \gets$ agent in $N_1$ with the highest value for $S_\ell$
	   \If{$v_a(S_\ell) \ge \beta$} 
	      \State $A_a\gets S_\ell$;\ $N \gets N \setminus \{a\}$;\ $M\gets M\setminus S_\ell$
	   \Else 
	      \State $a\gets$ agent in $N_2$ such that $v_a(S_\ell) \ge 3/4$
	   	 \State $A_a\gets S_\ell$;\ $N \gets N \setminus \{a\}$;\ $M\gets M\setminus S_\ell$    
	   \EndIf
	   \State $S_1\gets \{1\}$;\ \ $S_2\gets \{|N|, |N|+1\}$;\ \ $S_3\gets \{2|N|-1, 2|N|, 2|N|+1\}$;\ \ $S_4\gets\{1, 2|N|+1\}$
	   \State $T_1 \gets \{i\in N_1: \exists k\in [4], v_i(S_k) \ge \beta\}$; \ \ $T_2 \gets \{i\in N_2: \exists k\in [4], v_i(S_k) \ge 3/4\}$
  \EndWhile
  \State $n'\gets$ $|N_1 \cup N_2|$
  \State $R\gets$ $M\setminus [2n']$
  \State Initialize $n'$ bags as in \eqref{eq:B_i}
  \For{each $B_k, k\in [n']$} \Comment{Bag Filling}
  	\State $T \gets \{i\in N_1: v_i(B_k) \ge \beta\} \cup \{i\in N_2: v_i(B_k) \ge 3/4\}$
  	\While{$T = \emptyset$}
	  \State $B_k \gets B_k \cup \{g\}, g\in R$;\ $R\gets R\setminus \{g\}$ 
       \State $T \gets \{i\in N_1: v_i(B_k) \ge \beta\} \cup \{i\in N_2: v_i(B_k) \ge 3/4\}$
	\EndWhile
	  \State $a \gets$ agent in $N_1$ with the highest value for $B_k$
	  \If{$v_a(B_k) \ge \beta$} 
	     \State $A_a\gets B_k$;\ $N_1 \gets N_1 \setminus \{a\}$
	  \Else 
	     \State $a\gets$ agent in $N_2$ such that $v_a(B_k) \ge 3/4$ \Comment{$a$ exists due to while condition}
	     \State $A_a\gets B_k$;\ $N_2 \gets N_2 \setminus \{a\}$
	  \EndIf
  \EndFor
\end{algorithmic}
\end{algorithm}


In the bag filling phase, $n'$ bags are initialized using the first $[2n']$ goods as in~\eqref{eq:B_i} and each bag is filled with goods in $[m']\setminus [2n']$ until some agent has a value at least $3/4$ for the bag. Although the GT algorithm is quite simple, the main challenge is showing there are enough goods in $[m']\setminus [2n']$ to satisfy each agent with a value of at least $3/4$.

Our algorithm is described in Algorithm~\ref{algo:or}. We start with an arbitrary set $N_1$ of agents such that $|N_1|\le 2n(1-\beta)/\beta$, and our goal is to satisfy each of them with a value of at least $\beta$. $N_2$ is the set of remaining agents, and our goal is to satisfy each of them with a value of at least $3/4$. Like the GT algorithm, Algorithm~\ref{algo:or} also has two phases, valid reductions and bag filling, albeit with some crucial differences. In the valid reduction phase, we use different targets for $N_1$ and $N_2$, but we prioritize agents in $N_1$. We first check if a valid reduction is feasible for an agent in $N_1 \cup N_2$ with some $S_k, k\in[4]$. If yes, we pick the smallest feasible index, say $S_\ell$, and find an agent, say $a$, in $N_1$ with the highest value for $S_\ell$. If this value is at least $\beta$, we assign $S_\ell$ to agent $a$. Otherwise, we assign $S_\ell$ to any agent in $N_2$ with a value of at least $3/4$. 

We run the bag-filling phase on the reduced instance if no valid reductions are feasible. This phase is similar to the GT algorithm except that we again use different targets for agents in $N_1$ and $N_2$ and prioritize agents in $N_1$. For all $i \in [n']$, let $B_i$ be the $i^{\text{th}}$ initial bag (i.e., $B_i=\{i,2n'-i+1\}$) and $\hat{B}_i$ be the bag at the end of the algorithm (i.e., after the bag-filling phase).

Although Algorithm~\ref{algo:or} is a simple extension of the GT algorithm, the analysis is not straightforward because $S_4$ is not a valid reduction for $N_1$. We first show that each agent in $N_2$ will receive a bag valued at least $3/4$ at the end of the algorithm. 

%The next two lemmas show that all agents are satisfied with their respective targets, proving the algorithm's correctness.

\begin{lemma}\label{lem:N2}
Each agent in $N_2$ receives a bag valued at least $3/4$.
\end{lemma}

\begin{proof}
It easily follows from the GT algorithm because valid reductions do not decrease the MMS value of any remaining agent in $N_2$, and the bag filling does not add goods from $[m']\setminus [2n']$ to a bag when some agent in $N_2$ has a value at least $3/4$. 
\end{proof}

In the rest of the section, we show the following claim, proving the algorithm's correctness. 

\begin{lemma}\label{lem:n1}
Each agent in $N_1$ receives a bag valued at least $\beta$.
\end{lemma}

For a contradiction, suppose the bag filling phase stopped at iteration $k\le n'$ because $[m']\setminus [2n']$ is empty and an agent $a\in N_1$ has not received a bag. Since no more valid reductions are feasible, like in Corollary~\ref{cor:val}, we must have 
\begin{equation}
v_a(j) < \begin{cases} \beta & \forall j\le n'\\ \beta/2 & \forall n' < j \le 2n'\\ \beta/3 & \forall j> 2n' \end{cases}
\end{equation}

This implies that at the beginning of the bag filling phase, 
\begin{equation}\label{eqn:bk}
v_i(B_k) < 3\beta/2, \forall k\in [n']. 
\end{equation}
Further, if $\hat{B} \neq B_k$ for some $k$, then $v_a(\hat{B}) < \beta + \beta/3 = 4\beta/3$ for the bags assigned to other agents before iteration $k$ because $v_a(\hat{B}\setminus g) < \beta$, where $g$ is the last good added to $\hat{B}$ and $v_a(g) \le v_a(2n'+1) < \beta/3$. Also, $v_a(\hat{B}) < \beta$ for all bags assigned to agents in $N_2$ because we prioritize agents in $N_1$. Therefore, in the bag-filling phase, we have

\begin{equation}\label{eqn:hbk}
v_a(\hat{B}) < \begin{cases} \beta  & \text{ if } \hat{B} \text{ is assigned to an agent in } N_2\\
3\beta/2  & \text{ if } \hat{B} \text{ is assigned to an agent in } N_1  \end{cases}.
\end{equation}

During valid reductions, since we prioritize agents in $N_1$, we have 
\begin{equation}
v_a(S_{\ell}) < \beta \ \  \text{ if } S_{\ell} \text{ is assigned to an agent in } N_2 .
\end{equation}

We next bound the value of $v_a(S_{\ell})$ when it is assigned to an agent in $N_1$. We have 
\begin{equation}\label{eqn:sn1}
\begin{aligned}
v_a(S_1) & \le  1 \text{ for any reduction using } S_1 \text{ since the instance is $n$-normalized}\\
v_a(S_3) & <  3\beta/2 \text{ for any reduction using } S_3 \text{ since $S_2$ is not feasible} \\
v_a(S_4) & <  \beta + \beta/3 = 4\beta/3 \text{ for any reduction using } S_4 \text{ since $S_1$ and $S_3$ are not feasible}
\end{aligned}
\end{equation}

The only case left is reduction using $S_2$, for which we break the analysis into multiple cases. Let $S_{\ell_1}S_{\ell_2} \cdots$ for $\ell_i \in [4]$ be a series of reduction. Now, consider the transitions to $S_2$, i.e., $\cdots S_{\ell}[S_2]^{t}S_{\ell'}\cdots$, where $\ell,\ell' \neq 2$ and $t\ge 1$ denote the number of $S_2$'s between $S_{\ell}$ and $S_{\ell'}$. Let $S_2^{t'}$ denote the $t'$-th $S_2$ for $t'\in [t]$. There are three cases: 
\smallskip

\textbf{Case 1} $[S_1]^{s}[S_2]^{t}\cdots:$ Here, $S_1$ occurs exactly $s\ge 0$ times. This case can happen at most once since $S_1$'s are the highest priority, and once $S_1$ is not feasible, it remains infeasible. 
%\HA{$S_2$ is a valid reduction before any $S_4$ happens. So in Case 1, $v_a(S_2^{t'}) \leq 1$.}
\begin{lemma}[Case 1]\label{lem:s1}
$v_a(S_2^{t'}) < 3\beta/2, \forall t'\in [t]$. 
\end{lemma}

\begin{proof}
Note that $S_2^{t'} := \{n-t'+1,n+t'\}, \forall t'\in [t]$, where $n$ is the number of agents in the original instance. By the pigeonhole principle, a bundle in $a$'s MMS partition $P^a$ must contain two goods from $[n+1]$. This, together with the instance being $n$-normalized, implies that $v_{a}(S_2^1) \le 1$. For $t'\ge 2$, if $v_a(S_2^{t'}) > 1$, then the goods in $\{n-t'+2, \dots, n+t'\}$ must be in $t'-1$ different bundles in $P^a$, which implies that there must be a bundle in $P^a$ that contains at least three goods from $\{n-t'+2, \dots, n+t'\}$ by the pigeonhole principle. This further implies that $v_a(n+t') \le 1/3$ because the instance is $n$-normalized. 

Finally, since $S_1$ is not feasible when the algorithm performs $S_2$, we have $v_a(n-t'+1) < \beta, \forall t' \in [t]$ and then we have $v_a(S_2^{t'}) = v_a(n-t'+1) + v_a(n+t') < \beta + 1/3 < 3\beta/2, \forall t'\ge 2$ using $\beta>3/4$. 
\end{proof}

\textbf{Case 2} $\cdots S_4[S_2]^{t}\cdots$: This case cannot happen because $S_2$ was not feasible when $S_4$ was performed and the set of goods in $S_2$ doesn't change after an $S_4$. 
\medskip

\textbf{Case 3} $\cdots S_3[S_2]^{t}\cdots$: Let $s$ be the number of agents just before the instance is reduced using $S_3$, which implies that $S_3 = \{2s+1, 2s, 2s-1\}$ and $S_2 = \{s-1, s\}$. Let $x:= v_a(S_3)$, which implies that $v_a(2s-1) \ge x/3$. Since $S_2$ is not feasible when we used $S_3$, we have $v_a(\{s, s+1\}) < \beta$, which further implies that $x<3\beta/2$. Furthermore, we have $v_a(s+1) \ge v_a(2s-1) \ge x/3$ and $v_a(s) < \beta - x/3$. Next, we break the analysis into two subcases depending on whether there are more $S_3$ reductions later. 

\textbf{Case 3a:} If this is the last reduction with $S_3$, then we have $v_a(\{s-1, s\} < \beta + \beta - x/3 < 2\beta$. Since all later $S_2 = \{j, j'\}$'s will have a $j<s-1$ and $j'>s+1$, we have $v_a(\{j, j'\}) < \beta + \beta/2 = 3\beta/2$ for each of them. Note that this case can occur at most once. 

\textbf{Case 3b:} For the other case, if this is not the last $S_3$, then we must have $v_a(\{s-2, 2s-2\})<\beta$ otherwise, $S_2$ will always be feasible contradicting the fact that this is not the last $S_3$. This implies that $v_a(s-1) \le v_a(s-2) < \beta - v_a(2s-2) < \beta - x/3$.  Then, we have 
$$v_a(S_2^1 \cup S_3) = v_a(\{s-1, s\}) + v_a(S_3) < 2\beta - 2x/3 + x < 2\beta + x/3 < 5\beta/2.$$
Furthermore, for each of the remaining $t-1$ $S_2 = \{j, j'\}$'s, we have $j<s, j'>s$, implying $v_a(\{j, j'\} < \beta + \beta/2 = 3\beta/2$. 
The above analysis implies that 

\begin{corollary}
In Case 3, either $v_a(S_2^1 \cup S_3) < 5\beta/2$ or $v_a(S_2^1) < 2\beta$. For the remaining $t-1$ $S_2$'s, $v_a(S_2^{t'}) < 3\beta/2, \forall t'\ge 2$. 
\end{corollary}

We are now ready to prove Lemma~\ref{lem:n1}.

\begin{proof}(of Lemma~\ref{lem:n1})
Recall that we assumed for a contradiction that the bag filling phase stopped at iteration $k\le n'$ because $[m']\setminus [2n']$ is empty and an agent $a\in N_1$ has not received a bag. Lemma~\ref{lem:N2} implies that all agents in $N_2$ must have received a bag valued at least $3/4$ before this iteration. 

Since we prioritize agents in $N_1$ in both valid reductions and bag filling, we have $v_a(S) < \beta$ whenever $S$ is given to an agent in $N_2$. Further, \eqref{eqn:bk} and \eqref{eqn:hbk} imply that both $v_a(B_k)$  and $v_a(\hat{B})$ are strictly less than $3\beta/2$ at the beginning and when assigned to other agents in the bag filling phase. In valid reductions, except for Case 3 of $S_2$, \eqref{eqn:sn1} and Lemma~\ref{lem:s1} imply that $v_a(S_\ell) < 3\beta/2$. Case 3a of $S_2$ occurs at most once, which implies that for all $S_2$'s in this case except for one, say $S_2^*$, we have $v_a(S_2) < 3\beta/2$ and $v_a(S_2^*) < 2\beta$. Case 3b of $S_2$ implies that $v_a(S_3 \cup S_2^1) < 5\beta/2$ and for all other $S_2$'s we have $v_a(S_2) < 3\beta/2$. Therefore, we have

\begin{equation}\nonumber
\begin{aligned}
n = v_a(M) & = \sum_{S \text{ assigned to } i\in N_2} v_a(S) + \sum_{S \text{ assigned to } i\in N_1} v_a(S) + v_a(B_k) + \sum_{j=k+1}^{n'} v_a(B_j)\\
& < \beta\cdot (3\beta-2)n/\beta + 3\beta/2\cdot (2(1-\beta)n/\beta-(n'-k+2)) + 2\beta + v_a(B_k) + 3\beta/2\cdot (n'-k)\\
& = n - \beta + v_a(B_k), 
\end{aligned}
\end{equation}
which implies that $v_a(B_k) > \beta$, a contradiction. 
\end{proof}



==> missing-proofs.tex <==
\section{Missing Proofs of Section \ref{sec:4n-3}}\label{missing-proofs-4n-3}
\upperBoundLeft*
\begin{proof}
    Let $g$ be the good with the largest index in $\hat{B}_j$. If $g = 2n-j+1$, $v_i(\hat{B}_j \setminus \{g\}) = v_i(j)  \leq 1$ by Proposition \ref{prop:exact}(\ref{exact:1}). If $g > 2n-j+1$, meaning that $g$ was added to $\hat{B}_j$ during bag-filling, then $v_i(\hat{B}_j \setminus \{g\}) < 1$. Otherwise, $g$ would not be added to $\hat{B}_j$. Therefore,
    \begin{align*}
        v_i(\hat{B_j}) &= v_i(\hat{B}_j \setminus \{g\}) + v_i(g) \\
        &\leq 1 + v_i(2n-k+1). &\tag{$v_i(\hat{B}_j \setminus \{g\}) \leq 1$ and $g \geq 2n-k+1$}
    \end{align*}
\end{proof}

\upperBoundRight*
\begin{proof}
    First, assume $\hat{B}_j \neq B_j$ and $g$ be the last good added to $\hat{B}_j$. We have $v_i(\hat{B}_j \setminus \{g\}) < 1$. Otherwise, $g$ would not be added to $\hat{B}_j$. Therefore,
    \begin{align*}
        v_i(\hat{B_j}) &= v_i(\hat{B}_j \setminus \{g\}) + v_i(g) \\
        &< 1 + v_i(2n-k+1). &\tag{$v_i(\hat{B}_j \setminus \{g\}) < 1$ and $g > 2n-k+1$}
    \end{align*}
    Now assume $\hat{B}_j = B_j$. We have
    \begin{align*}
        v_i(\hat{B}_j) &= v_i(B_j) \\
        &= v_i(j) + v_i(2n-j+1) \\
        &\leq 2v_i(k). &\tag{$2n-j+1 > j \geq k$}
    \end{align*}
    Hence, $v_i(\hat{B}_j) \leq \max(1 + v_i(2n-k+1), 2v_i(k))$.
\end{proof}

\lessThanOne*
\begin{proof}
    Otherwise, the algorithm would allocate the remaining bag with the smallest index to agent $i$.
\end{proof}

\noChange*
\begin{proof}
    For all $B_j \in A^+$, $v_i(B_j) \geq 1$. Since $i$ did not receive any bundle, $B_j$ must have been assigned to some other agent, and no good needed to be added to $B_j$ in bag-filling since there is an agent (namely $i$) with no bag who values $B_j$ at least $1$.
\end{proof}

\halfBound*
\begin{proof}
    Since $v_i(B_{\ell^*+1}) = v_i(\ell^*+1)+ v_i(2n-\ell^*) < 1$ and $v_i(2n-\ell^*) \leq v_i(\ell^*+1)$, $v_i(2n-\ell^*) < 1/2$.
    Also for all $j \geq 2n-\ell^*$, $v_i(j) \leq v_i(2n-\ell^*) < 1/2$.
\end{proof}

\sGl*
\begin{proof}
    For all $j < \ell^*$, $v_i(B_{j+1}) \geq 1$. Since $i$ did not receive any bundle, $B_{j+1}$, must have been assigned to another agent. Therefore, the algorithm does not stop at step $j+1$. Also, by Observation \ref{no-change}, $B_{j+1}$ gets no good in bag-filling.
\end{proof}

\saveTwo*
\begin{proof}
    We have
    \begin{align*}
        1 > v_i(B_{\ell^*+1}) = v_i(\ell^*+1) + v_i(2n-\ell^*) = v_i(\ell^*+1) + \frac{1}{3} + x.
    \end{align*}
    Hence, $v_i(\ell^*+1) < 2/3 - x$. Also, for $B_j \in A^2$, we have
    \begin{align*}
        v_i(B_j) &= v_i(j) + v_i(2n-j+1) \\
        &\leq 2v_i(\ell^*+1) &\tag{$2n-j+1 > j \geq \ell^*+1$ since $B_j \in A^2$} \\
        &< \frac{4}{3} - 2x.
    \end{align*}
    So if $\hat{B}_j = B_j$, the inequality holds. Now assume $\hat{B}_j \neq B_j$. This implies that $j \geq s+1$ and the algorithm did not stop at step $j$ before adding a good to $B_j$. Therefore it did not stop at step $s +1$ before adding a good to $B_{s+1}$ either. Let $g$ be the first good added to $B_{s+1}$. Since $B_{s+1}$ requires more than one good,
    \begin{align*}
        1 > v_i(B_{s +1} \cup \{g\}) &= v_i(s+1) + v_i(n-s) + v_i(g) \\
        &\geq 2v_i(2n-\ell^*) + v_i(g) &\tag{$s+1 < n-s \leq 2n-\ell^*$} \\
        &= \frac{2}{3} + 2x + v_i(g).
    \end{align*}
    Therefore, $v_i(g) < 1/3 - 2x$. Now let $h$ be the last good added to bag $B_j$. We have
    \begin{align*}
        v_i(\hat{B}_j) &= v_i(\hat{B}_j \setminus \{h\}) + v_i(h) \\
        &< 1 + v_i(g) &\tag{$v_i(\hat{B}_j \setminus \{h\}) < 1$ and $v_i(h) \leq v_i(g)$} \\
        &< \frac{4}{3} - 2x. \qedhere
    \end{align*}
\end{proof}


\saveAll*
\begin{proof}
    First assume $B_j \in A^+$. We have $j \leq \ell^*$. Also,
    \begin{align*}
        v_i(\hat{B}_j) &= v_i(B_j) &\tag{$\hat{B}_j = B_j$} \\
        &= v_i(j) + v_i(2n-j+1) \\
        &\leq 1 + v_i(2n-\ell^*) &\tag{$v_i(j) \leq 1$ and $2n-j+1 > 2n-\ell^*$} \\
        &= \frac{4}{3} +x.
    \end{align*}
    Now assume $B_j \in A^1$. Let $g$ be the good added to bag $B_j$ in bag-filling. We have,
    \begin{align*}
        v_i(\hat{B}_j) &= v_i(B_j) + v_i(g) \\
        &< 1 + v_i(2n-\ell^*) &\tag{$v_i(B_j) < 1$ and $v_i(g) \leq v_i(2n+1) \leq v_i(2n-\ell^*)$}\\
        &= \frac{4}{3} + x. \qedhere
    \end{align*}
\end{proof}

\begin{lemma}\label{r-star-bound}
    If $v_i(2n-r^*+1) \leq 1/3$, then $r^* < 2n/3$.
\end{lemma}
\begin{proof}
    Since $1>v_i(B_{r^*})=v_i(r^*)+v_i(2n-r^*+1)$, we have $v_i(r^*)<2/3+x$.
    By Observation \ref{upper-bound-left}, for all $j \leq r^*$, $v_i(\hat{B}_j) \leq 4/3-x$.
    Also, by Observation \ref{upper-bound-right}, for all $j>r^*$, $v_i(\hat{B}_j)<4/3+2x$.
    Hence, we have
    \begin{align*}
        \frac{4n}{3} &= v_i(M) \\
        &= \sum_{j \leq r^*} v_i(\hat{B}_j) + \sum_{j > r^*} v_i(\hat{B}_j) \\
        &< r^*(\frac{4}{3}-x) + (n-r^*)(\frac{4}{3}+2x) \\%&\tag{Corollary \ref{cor-r-star} and \ref{claim-r-star-1}}\\
        &= \frac{4n}{3} + x(2n-3r^*).
    \end{align*}
    Therefore, $r^* < 2n/3$.
\end{proof}

\rStarLemma*
\begin{proof}
    Towards contradiction, assume $v_i(2n-r^*+1) = 1/3-x$ for $x \geq 0$. By Lemma \ref{r-star-bound}, $r^* < 2n/3$.
    \begin{claim}\label{claim-r-star}
        $\sum_{j > r^*} v_i(\hat{B}_j) < \frac{10n}{9}-r^* + \frac{2nx}{3}$.
    \end{claim}
    \begin{claimproof}
    Note that by the definition of $r^*$, for all $j > r^*$, $\hat{B}_j = B_j$.
    By Lemma \ref{lem:Csum}, $v_i(\{2n/3+r^*+1, \ldots, 2n-r^*\}) \leq 2n/3-r^*$. Also since $v_i(r^*) < 2/3+x$, $v_i(\{r^*+1, \ldots, 2n/3+r^*\}) \leq \frac{2n}{3}(\frac{2}{3}+x)$. In total, we get
    \begin{align*}
        \sum_{j > r^*} v_i(\hat{B}_j) &= \sum_{j > r^*} v_i(B_j) \\
        &= v_i(\{r^*+1, \ldots, 2n/3+r^*\}) + v_i(\{2n/3 +r^*+1, \ldots, 2n-r^*\}) \\
        &< \frac{2n}{3}(\frac{2}{3}+x) + \frac{2n}{3}-r^* \\
        &= \frac{10n}{9}-r^* + \frac{2nx}{3}.
    \end{align*}
    Therefore, Claim \ref{claim-r-star} holds.
    \end{claimproof}
    We have
    \begin{align*}
        \frac{4n}{3} &= v_i(M) \\
        &= \sum_{j \leq r^*} v_i(\hat{B}_j) + \sum_{j > r^*} v_i(\hat{B}_j) \\
        &< r^*(\frac{4}{3} -x) + \frac{10n}{9}-r^* + \frac{2nx}{3} &\tag{Observation \ref{upper-bound-left} and Claim \ref{claim-r-star}}\\
        &= r^*(\frac{1}{3}-x) + \frac{10n}{9} + \frac{2nx}{3}.
    \end{align*}
    Thus,
    \begin{align*}
        \frac{2n}{9} &< r^*(\frac{1}{3}-x) + \frac{2n}{3}(x) \\
        &\leq \frac{2n}{3} \cdot \frac{1}{3}, \tag{$r^* \leq 2n/3$ by Lemma \ref{r-star-bound}}
    \end{align*}
    which is a contradiction. Hence, $v_i(2n-r^*+1) > 1/3$.
\end{proof}

\begin{restatable}{observation}{lessThanThree}\label{lessThan13}
    $x < 1/3$.    
\end{restatable}
\begin{proof}
    Towards a contradiction, assume $x=1/3$. Therefore, $v_i(2n-\ell+1)=0$. Let $k < 2n-\ell+1$ be the number of goods with a value larger than $0$ to agent $i$. Consider $(P^i_1 \cap [k], \ldots, P^i_{4n/3} \cap [k])$. There are at least $\ell$ many indices $j$ such that, $|P^i_j \cap [k]|=1$. Since $\mathcal{I}$ is $4n/3$-normalized, $v_i(1) = \ldots = v_i(\ell)=1$ which is a contradiction with $v_i(B_{\ell^*+1})<1$.
\end{proof}

\begin{restatable}{observation}{yBound}\label{y-bound}
    $y< 1/6$.    
\end{restatable}
\begin{proof}
    We have $1/3 + y = v_i(2n-r) \leq v_i(B_r)/2 < 1/2$. Thus, $y<1/6$.
\end{proof}

\middleBlock*
\begin{proof}
    Note that by definition of $\ell$ and $r$, for all $\ell < j \leq r$, $v_i(B_j) \geq 1$. Therefore, $\hat{B}_j=B_j$. Also,
    \begin{align*}
        v_i(B_j) &= v_i(j) + v_i(2n-j+1) \\
        &\leq v_i(\ell) + v_i(2n-r) \tag{$\ell < j$ and $2n-r < 2n-j+1$}\\
        &< (\frac{2}{3}+x) + (\frac{1}{3}+y) \tag{$v_i(B_\ell)<1$ and $v_i(B_{r+1})<1$}\\
        &= 1+x+y.
    \end{align*}
\end{proof}

\rMinusl*

\thmOneoodHard*
\begin{proof}
$u$ is ordered since $u(2n) = u(2n+1) = 1/3$.

Define $M \defeq (M_1, \ldots, M_d)$ as
\[ M_i \defeq \begin{cases}
\{i, 2n-1-i\} & \textrm{ if } 1 \le i \le n-1
\\ \{i+n-1, 2d+n-i, 2d-n+i+1\} & \textrm{ if } n \le i \le d
\end{cases}. \]
To show that $u$ is normalized, we show that $u(M_i) = 1$ for all $i \in [d]$.
For $i \in [n-1]$, we have
\begin{align*}
u(M_i) &= u(i) + u(2n-1-i) = \frac{4}{3} - \frac{\ceil{i/2} + \ceil{(2n-1-i)/2}}{3n}
\\ &= 1 - \frac{\ceil{i/2} + \ceil{-(i+1)/2}}{3n} = 1.
\end{align*}
For $i \in [d] \setminus [n-1]$ and $g \in M_i$, we have $g \ge 2n-1$.
Since $u(j) = 1/3$ for all $j \ge 2n-1$, we get that $u(M_i) = 1$ for $i \in [d] \setminus [n-1]$.
\end{proof}

\thmOneoodHardOutput*
\begin{proof}
For $i \in [n]$, let $B_i \defeq \{i, 2n+1-i\}$ be the initial bag. Then
\begin{align*}
u(B_i) &= u(i) + u(2n+1-i) = \frac{4}{3} - \frac{\ceil{i/2} + \ceil{(2n+1-i)/2}}{3n}
\\ &= \frac{4}{3} - \frac{(n+1) + \ceil{i/2} + \ceil{-(i+1)/2}}{3n}
= 1 - \frac{1}{3n}.
\end{align*}
Since $m-2n \le n-1$ goods are left after bag initialization, and each good has value $1/3$,
the first $m-2n$ bags get 1 good each during bag filling,
and the remaining bags do not get any goods.
\end{proof}


\subsection{Proof of Lemma \ref{expowerful}}\label{lemma-expowerful-proof}
To prove Lemma \ref{expowerful}, we partition the goods considered in this lemma into two parts. These parts are colored red and blue in Figure \ref{colorful-1}. We bound the value of red goods in Lemma~\ref{k-t}, i.e.,
\[ \sum_{2n-\ell^* < j\leq 2n-t}v_i(j) + \sum_{8n/3 - 2\ell-t-2\ell^* < j \leq 8n/3 - 2\ell - 2t - \ell^*}v_i(j) < \ell^*-t, \]
and the value of the blue goods in Lemma~\ref{k+l}, i.e.,
\[ \sum_{t < j \leq \ell^*} v_i(j) + \sum_{8n/3 - 2\ell - 2t - \ell^* < j \leq 8n/3 + \ell}v_i(j) \leq \ell^* + \ell. \]
Thereafter, we have
\begin{align*}
    v_i(&\{8n/3 - 2\ell-t-2\ell^*+1, \ldots, 8n/3 + \ell\} \\
    &\cup \{t+1, \ldots, \ell^*\} \\
    &\cup \{2n-\ell^*+1, \ldots, 2n-t\}) \\
    &= \textcolor{red}{\sum_{2n-\ell^* < j\leq 2n-t}v_i(j) + \sum_{8n/3 - 2\ell-t-2\ell^* < j \leq 8n/3 - 2\ell - 2t - \ell^*}v_i(j)} \\
    &+ \textcolor{blue}{\sum_{t < j \leq \ell^*} v_i(j) + \sum_{8n/3 - 2\ell - 2t - \ell^* < j \leq 8n/3 + \ell}v_i(j)} \\
    &< (\ell^*-t) + (\ell^*+\ell) &\tag{Lemma \ref{k-t} and \ref{k+l}}\\
    &= 2\ell^*+\ell-t,
\end{align*}
and Lemma \ref{expowerful} follows.

It suffices to prove Lemmas \ref{k-t} and \ref{k+l}. In the rest of this section, we prove these two lemmas.
\begin{figure}[!hbt]
    \centering
    \scalebox{\figScale}{\input{figs/Lemma-Fig.tikz}}
    \captionAndDescr{The goods considered in in Lemma~\ref{k-t} are marked with red and the goods in Lemma~\ref{k+l} are marked with blue.}
    \label{colorful-1}
\end{figure}
Limit the goods in a $1$-out-of-$4n/3$ MMS partition of agent $i$ to $\{1, \ldots, 8n/3+\ell\}$ and let $R$ be the set of the resulting bags. Formally, for all $j \in [4n/3]$, $R_j = P_j^{i} \cap \{1, \ldots, 8n/3+\ell\}$ and $R = \{R_1, \ldots, R_{4n/3}\}$. Without loss of generality, assume $|R_1| \geq |R_2| \geq \ldots \geq |R_{4n/3}|$. Let $t$ be the number of bags of size $1$ in $R$.

\begin{lemma}\label{powerful}
    If there exist $t$ bags of size at most $1$ in $R$, then
    \[ \sum_{1 \leq j \leq t+\ell}|R_j| \geq 3(t+\ell). \]
\end{lemma}
\begin{proof}
    Since $R_j$'s are sorted in decreasing order of their size,
    \begin{align*}
        \sum_{1 \leq j \leq t+\ell}|R_j| \geq (t+\ell)|R_{t+\ell}|.
    \end{align*}
    Hence, if $|R_{t+\ell}| \geq 3$, then $\sum_{1 \leq j \leq t+\ell}|R_j| \geq 3(t+\ell).$ So assume $|R_{t+\ell}| \leq 2$.
    \begin{align*}
        \frac{8n}{3} + \ell &= \sum_{1 \leq j \leq 4n/3}|R_j| \\
        &= \sum_{1 \leq j \leq t+\ell} |R_j| + \sum_{t+\ell < j \leq 4n/3 - t}|R_j| + \sum_{4n/3-t < j \leq 4n/3}|R_j| \\
        &\leq \sum_{1 \leq j \leq t+\ell} |R_j| +  (\frac{4n}{3} - 2t - \ell)|R_{t+\ell}| + t \\
        &\leq \sum_{1 \leq j \leq t+\ell} |R_j| + 2(\frac{4n}{3} - 2t - \ell) + t
    \end{align*}
    Therefore, \[ \sum_{j \in [t+\ell]} |R_j| \geq 3(\ell+t). \]
\end{proof}
\begin{lemma}\label{bound}
    $\ell+\ell^*+t \leq 4n/3$.
\end{lemma}
\begin{proof}
    We have $\ell^* + 2n/3 + \ell \leq s \leq n$. See Figure \ref{colorful} for intuition. Therefore, $\ell^* + \ell \leq n/3$. Also, $t \leq \ell^* \leq n$. Hence $\ell+\ell^*+t \leq 4n/3$.
\end{proof}
\begin{lemma}\label{k-t}
    \textcolor{red}{
    \[ \sum_{2n-\ell^* < j\leq 2n-t}v_i(j) + \sum_{8n/3 - 2\ell-t-2\ell^* < j \leq 8n/3 - 2\ell - 2t - \ell^*}v_i(j) < \ell^*-t. \]
    }
\end{lemma}
\begin{proof}
    Let $B' = \{2n-\ell^*+1, \ldots, 2n-t\} \cup \{8n/3 - 2\ell-t-2\ell^*+1, \ldots, 8n/3 - 2\ell - 2t - \ell^*\}$. $|B'| = 2(\ell^*-t)$ and by Observation \ref{half-bound} for all goods $g \in B'$, $v_i(g) < 1/2$. Therefore, $v_i(B') < \ell^*-t$.
\end{proof}
\begin{lemma}\label{k+l}
    \textcolor{blue}{
\[ \sum_{t < j \leq \ell^*} v_i(j) + \sum_{8n/3 - 2\ell - 2t - \ell^* < j \leq 8n/3 + \ell}v_i(j) \leq \ell^* + \ell. \]
    }
\end{lemma}
\begin{proof}
    Recall that $\{R_1, \ldots, R_{4n/3}\}$ is the set of bags in the $1$-out-of-$4n/3$ MMS partition of agent $i$ after removing goods $\{8n/3+\ell+1, \ldots, m\}$. Moreover, we know exactly $t$ of these bags have size $1$. If there is a bag $R_j = \{g\}$ for $g>t$, there must be a good $g' \in [t]$ such that $g' \in R_{j'}$ and $|R_{j'}|>1$. Swap the goods $g$ and $g'$ between $R_j$ and $R_{j'}$ as long as such good $g$ exists. Note that $v_i(R_{j'})$ can only decrease and $v_i(R_j)=v_i(g') \leq 1$. Therefore, in the end of this process for all $j \in [4n/3]$, $v_i(R_j) \leq 1$ and we can assume bags containing goods $1, \ldots, t$ are of size $1$ and bags containing goods $t+1, \ldots, \ell^*$ %\jnote{here what is $k$? should it be $8n/3 + \ell$?}
    are of a size more than $1$. Recall that $|R_1| \geq \ldots \geq |R_{4n/3}|$. Let $T_{j}$ be the bag that contains good $j$.

    Consider the bags $B=\{R_1, \ldots, R_{t+\ell}\} \cup \{T_{t+1}, \ldots, T_{\ell^*}\}$. If $|B| < \ell^*+\ell$, keep adding a bag with the largest number of goods to $B$ until there are exactly $\ell^*+\ell$ bags in $B$. First we show that $B$ contains at least $3\ell + 2\ell^* + t$ goods. Namely,
    \[ \sum_{S \in B} |S| \geq 3\ell + 2\ell^* + t. \]
    By Lemma \ref{powerful}, $\sum_{1 \leq j \leq t+\ell} |R_j| \geq 3(t+\ell)$. If all the remaining $\ell^*-t$ bags in $B \setminus \{R_1, \ldots, R_{t+\ell}\}$ are of size $2$, then $\sum_{S \in B} |S| \geq 3(t+\ell)+2(\ell^*-t) = 3\ell + 2\ell^* +t$. Otherwise, there is a bag in $B$ of size at most $1$; hence, all bags outside $B$ are also of size at most $1$. So we have
    \begin{align*}
        \frac{8n}{3} + \ell &= \sum_{S \in B} |S| + \sum_{S \notin B} |S| \\
        &\leq \sum_{S \in B} |S| + (\frac{4n}{3} - \ell^* - \ell).
    \end{align*}
    Therefore,
    \begin{align*}
        \sum_{S \in B} |S| &\geq 4n/3 + 2\ell + \ell^* \\
        &\geq 3\ell + 2\ell^* +t. &\tag{Lemma \ref{bound}}
    \end{align*}
    Note that the goods $\{t+1, \ldots, \ell^*\}$ are contained in $B$ and moreover, $B$ contains at least $3\ell + 2\ell^* +t - (\ell^*-t) = 3\ell + 2t + \ell^*$ other goods. Therefore,
    \begin{align*}
        \ell^*+\ell &\geq \sum_{S \in B} v_i(S) \\
        &\geq \sum_{t < j \leq \ell^*} v_i(j) + \sum_{8n/3 - 2\ell - 2t - \ell^* < j \leq 8n/3 + \ell} v_i(j).
    \end{align*}
The last inequality follows because we used the $3\ell + 2t + \ell^*$ lowest valued goods in $[8n/3+\ell]$.
\end{proof}


\subsection{Proof of Lemma \ref{difficult-bound}}\label{proof-sec-1}
The main idea is as follows. Recall that $s'=\min(|S'|,s)$. We consider two cases for $s'$. If $s' = s$, then in order to prove Lemma \ref{difficult-bound}, we must prove
\[ v_i(\{r-s'+1, \ldots, r\} \cup \{2n-\ell - s'+1, \ldots, 2n-\ell\}) \leq s', \]
which is what we do in Claim \ref{claim-2}.
In case $s' = |S'|$, we prove
\[ v_i(\{r-s'+1, \ldots, r\}) + v_i(S') \leq s' \]
in Claim \ref{claim-22} and
\[ v_i (\{2n-\ell-3s+2s'+1, \ldots, 2n-\ell\}) - v_i(S') \leq s-s' \]
in Claim \ref{claim-3}. Adding the two sides of the inequalities implies Lemma \ref{difficult-bound}. We prove this lemma in the rest of this section.

\difficultbound*
    Note that $\{1, \ldots, r\} \cup S' \subseteq P_1 \cup \ldots \cup P_r$.
    For $j \in [r]$, let $Q_j = P_j \cap (\{1, \ldots, r\} \cup S')$. We begin with proving the following claim. %\ref{claim-1}.
    \begin{claim}\label{claim-1}
        There are $s'$ many sets like $Q_{j_1}, \ldots, Q_{j_{s'}}$ such that $|\cup_{k \in [s']} Q_{j_k}| \geq 2s'$ and $|\cup_{k \in [s']} Q_{j_k} \cap \{1, \ldots, r\}| \geq s'$.
    \end{claim}
    \begin{proof}
        If $s'=0$, the claim trivially holds. Thus, assume $s' \geq 1$. By induction, we prove that for any $t \leq s'$, there are $t$ many sets like $Q_{j_1}, \ldots, Q_{j_t}$ such that $|\cup_{k \in [t]} Q_{j_k}| \geq 2t$ and $|\cup_{k \in [t]} Q_{j_k} \cap \{1, \ldots, r\}| \geq t$.
        \paragraph{\boldmath Induction basis: $t=1$.} If there exists $Q_k$ such that $|Q_k \cap \{1, \ldots, r\}| \geq 2$, let $j_1 = k$. Otherwise, for all $k \in [r]$, we have $|Q_k \cap \{1, \ldots, r\}| = 1$. Since $s' \geq 1$, there must be an index $k$ such that $|Q_k \cap S'| \geq 1$. Let $j_1=k$.

        \paragraph{\boldmath Induction assumption:} There are $t$ many sets like $Q_{j_1}, \ldots, Q_{j_t}$ such that $|\cup_{k \in [t]} Q_{j_k}| \geq 2t$ and $|\cup_{k \in [t]} Q_{j_k} \cap \{1, \ldots, r\}| \geq t$.

        Now for $t+1 \leq s'$, we prove that there are $t+1$ many sets like $Q_{j_1}, \ldots, Q_{j_{t+1}}$ such that $|\cup_{k \in [t+1]} Q_{j_k}| \geq 2t+2$ and $|\cup_{k \in [t+1]} Q_{j_k} \cap \{1, \ldots, r\}| \geq t+1$.
        \paragraph{\boldmath Case 1: $|\cup_{k \in [t]} Q_{j_k}| \geq 2t+2$:} If $|\cup_{k \in [t]} Q_{j_k} \cap \{1, \ldots, r\}| \geq t+1$, set $j_{t+1}=k$ for an arbitrary $k \in [r] \setminus \{j_1, \ldots, j_t\}$. Otherwise, set $j_{t+1}=k$ for an index $k \in [r] \setminus \{j_1, \ldots, j_t\}$ such that $|Q_{k} \cap \{1, \dots, r\}| \ge 1$.
        \paragraph{\boldmath Case 2: $|\cup_{k \in [t]} Q_{j_k}| = 2t+1$:} If there exists $k \in [r] \setminus \{j_1, \ldots, j_t\}$, such that $|Q_k \cap [r]| \geq 1$, set $j_{t+1}=k$. Otherwise, set $j_{t+1}=k$ for any $k \in [r] \setminus \{j_1, \ldots, j_t\}$ such that $|Q_k| \geq 1$. Since $|\cup_{j \in [r]} Q_j| \geq r+s' > 2t+1$, such $k$ exists.
        \paragraph{\boldmath Case 3. $|\cup_{k \in [t]} Q_{j_k}| = 2t$ and $|\cup_{k \in [t]} Q_{j_k} \cap \{1, \ldots, r\}| \geq t+1$:} $|\cup_{k \in [r] \setminus \{j_1, \ldots, j_t\}} Q_{j_k}| \geq r+s'-2t > r-t$. Therefore, by pigeonhole principle, there exists an index $k \in [r] \setminus \{j_1, \ldots, j_t\}$ such that $|Q_k| \geq 2$. Set $j_{t+1}=k$.
        \paragraph{\boldmath Case 4. $|\cup_{k \in [t]} Q_{j_k}| = 2t$ and $|\cup_{k \in [t]} Q_{j_k} \cap \{1, \ldots, r\}| = t$:} If there exists $k \in [r] \setminus \{j_1, \ldots, j_t\}$, such that $|Q_k \cap [r]| \geq 2$, set $j_{t+1}=k$. Otherwise, for all $k \in [r] \setminus \{j_1, \ldots, j_t\}$, $|Q_k \cap [r]|=1$ since $|\cup_{k \in [t]} Q_{j_k} \cap \{1, \ldots, r\}| = t$ and $|\cup_{k \in [r]} Q_{j_k} \cap \{1, \ldots, r\}| = r$. Set $j_{t+1}=k$ for any $k \in [r] \setminus \{j_1, \ldots, j_t\}$, such that $|Q_k \cap S'| \geq 1$. Since $|\cup_{j \in [r]} Q_j \cap S'| \geq s' > t$, such $k$ exists.
    \end{proof}
Now we prove Claim \ref{claim-2}.
\begin{claim}\label{claim-2}
    $v_i(\{r-s'+1, \ldots, r\} \cup \{2n-\ell - s'+1, \ldots, 2n-\ell\}) \leq s'$.
\end{claim}
\begin{proof}
    Let $Q^1$ be the set of $s'$ most valuable goods in $\cup_{k \in [s']} Q_{j_k}$ and let $Q^2$ be the set of $s'$ least valuable goods in $\cup_{k \in [s']} Q_{j_k}$. Since $|\cup_{k \in [s']} Q_{j_k}| \geq 2s'$, $Q^1 \cap Q^2 = \emptyset$. Also, $|\cup_{k \in [s']} Q_{j_k} \cap \{1, \ldots, r\}| \geq s'$. Thus, $v_i(Q^1) \geq v_i(\{r-s'+1, \ldots, r\})$. Moreover, $v_i(Q^2) \geq v_i(\{2n-\ell - s'+1, \ldots, 2n-\ell\})$. Hence,
    \begin{align*}
        s' &= \sum_{k \in [s']} v_i(P_{j_k}) \notag\\
        &\geq \sum_{k \in [s']} v_i(Q_{j_k}) \notag \\
        &\geq v_i(\{r-s'+1, \ldots, r\} \cup \{2n-\ell - s'+1, \ldots, 2n-\ell\}).
    \end{align*}
\end{proof}
Note that in case $s' = s$, Claim \ref{claim-2} implies Lemma \ref{difficult-bound}. Therefore, from now on, we assume $s' = |S'| < s$.
\begin{claim}\label{claim-22}
    $v_i(\{r-s'+1, \ldots, r\}) + v_i(S') \leq s'$.
\end{claim}
\begin{proof}
    The proof is similar to the proof of Claim \ref{claim-2}. Let $Q^1$ be the set of $s'$ most valuable goods in $\cup_{k \in [s']} Q_{j_k}$ and let $Q^2$ be the set of $s'$ least valuable goods in $\cup_{k \in [s']} Q_{j_k}$. Since $|\cup_{k \in [s']} Q_{j_k}| \geq 2s'$, $Q^1 \cap Q^2 = \emptyset$. Also, $|\cup_{k \in [s']} Q_{j_k} \cap \{1, \ldots, r\}| \geq s'$. Thus, $v_i(Q^1) \geq v_i(\{r-s'+1, \ldots, r\})$. Moreover, $v_i(Q^2) \geq v_i(S')$ since $s' = |S'|$. Hence,
    \begin{align*}
        s' &= \sum_{k \in [s']} v_i(P_{j_k}) \notag\\
        &\geq \sum_{k \in [s']} v_i(Q_{j_k}) \notag \\
        &\geq v_i(\{r-s'+1, \ldots, r\} \cup S')\\
        &= v_i(\{r-s'+1, \ldots, r\}) + v_i(S').
    \end{align*}
\end{proof}
\begin{claim}\label{claim-3}
    $v_i (\{2n-\ell-3s+2s'+1, \ldots, 2n-\ell\}) - v_i(S') \leq s-s'.$
\end{claim}
\begin{proof}
    Note that by definition of $S'$, the $2n-\ell-r-s'=8n/3-2r+s-s'$ goods in $\{r+1, \ldots, 2n-\ell\} \setminus S'$ are in $P_{r+1} \cup \ldots \cup P_{4n/3}$. Now for $j \in [4n/3 - r]$, let $R_j = P_{j+r} \cap \{r+1, \ldots, 2n-\ell\} \setminus S'$. Assume $|R_{j_1}| \geq \ldots \geq |R_{j_{4n/3-r}}|$. We prove
    \begin{align}
        \sum_{k \leq s-s'} |R_{j_k}| \geq 3(s-s'). \label{R-bound}
    \end{align}
    If $|R_{j_{s-s'+1}}| \geq 3$, Inequality \eqref{R-bound} holds. Otherwise, we have
    \begin{align*}
        \frac{8n}{3}-2r+s-s' &= \sum_{k \in [4n/3-r]} |R_{j_k}| \\
        &= \sum_{k \leq s-s'} |R_{j_k}| + \sum_{s-s' < k \leq 4n/3-r} |R_{j_k}| \\
        &\leq \sum_{k \leq s-s'} |R_{j_k}| + 2(\frac{4n}{3}-r-s+s'). \tag{$|R_{j_k}| \leq 2$ for $k > s-s'$}
    \end{align*}
    Thus, $\sum_{k \in [s-s']} |R_{j_k}| \geq 3(s-s')$. We have
    \begin{align*}
        s-s' &= \sum_{k \in [s-s']} v_i(P_{j_k+r}) \notag\\
        &\geq \sum_{k \in [s-s']} v_i(R_{j_k}) \notag\\
        &\geq v_i (\{2n-\ell-3s+2s'+1, \ldots, 2n-\ell\}) - v_i(S'). \tag{$\lvert \cup_{k \in [s-s']} R_{j_k} \rvert \geq 3(s-s')$ and $\lvert S' \rvert =s'$}
    \end{align*}
\end{proof}
Claims \ref{claim-22} and \ref{claim-3} imply Lemma \ref{difficult-bound}.

\section{Missing Proofs of Section \ref{sec:algo1}}\label{missing-proofs-2}
\thmRedn*
\begin{proof}
All type-1 reductions happen together in the beginning.
This is because a different kind of reduction can only happen if a type-1 reduction is not possible.
If a type-1 reduction is not possible, then for each good $g$ and each remaining agent $i$,
$v_i(g) < \tau_i$. Hence, a type-1 reduction will never happen in the future.

Call $R_i$ the $i\Th$ \emph{phase} of \ $\RBF$.
Within each phase, all type-2 reductions happen before all type-4 reductions.
This is because a type-4 reduction happens only if a type-2 reduction is not possible.
After a type-4 reduction, the value of $S_2$ remains the same,
so a type-2 reduction will never occur again in the same phase.
\end{proof}

\thmMGe*
\begin{proof}
Let $\Ical \defeq ([n], [m], \Vcal)$ be the initial fair division instance (the input to $\RBF$).

By \cref{thm:redn-seq}, all type-1 reductions happen before all other reductions.
Suppose $k$ type-1 valid reductions happened. Immediately after that,
$|M| = m - k$ and $|N| = n - k$. If $|M| < 2|N|$, then $m < 2n-k$.
For any agent $i \in [n]$, consider her partition $P \defeq (P_1, \ldots, P_n)$ for $\Ical$.
Since $m < 2n-k$, at least $k+1$ singleton bundles in $P$ exist.
Since $\Ical$ is normalized, the goods in those singleton bundles have a value of $1$ for $i$.
But at least $k+1$ type-1 reductions should have happened, which is a contradiction.
Hence, immediately after type-1 reductions, we have $|M| \ge 2|N|$.

Type-3 and type-4 reductions only happen when $|M| \ge 2|N|+1$,
so they preserve the invariant $|M| \ge 2|N|$.
\end{proof}

\thmRednVS*\begin{proof}
Suppose $p$ reductions happen during $\RBF$. For any $i \in [p]$,
let $S_i$ be the $i\Th$ reduction bundle and let $k_i$ be the type of the $i\Th$ reduction.
Let $M_i$ and $N_i$ be the set of remaining goods and remaining agents, respectively,
after $i$ reductions have happened. (Hence, $(N_0, M_0, \Vcal)$ is the original instance.)

Define proposition $P(i)$ as: For any $j \in [i]$ and any $g \in S_i$,
$g > \ordSt(M_i, |N_i|)$ if $k = 2$ and $g > \ordSt(M_i, 2|N_i|)$ if $k = 3$.

We prove $P(i)$ for all $i \in \{0\} \cup [p]$ using induction:
The base case $i = 0$ is trivial since no reductions have happened.
Now for $i \in [p]$, we want to prove $P(i-1) \implies P(i)$.

\textbf{Case 1}: $k_i = 1$:
\\ By \cref{thm:redn-seq}, no type-2 or type-3 reductions happened among the first $i$ reductions.
Hence, $P(i)$ holds trivially.

For the remaining cases, $\ordSt(M_i, |N_i|)$ and $\ordSt(M_i, 2|N_i|)$ are well-defined
because of \cref{thm:m-ge-2n}.

\textbf{Case 2}: $k_i = 2$:
\\ Then $S_i = \ordSt(M_{i-1}, \{|N_{i-1}|, |N_{i-1}|+1\})$,
$\ordSt(M_i, |N_i|) = \ordSt(M_{i-1}, |N_{i-1}|-1)$,
and $\ordSt(M_i, 2|N_i|) = \ordSt(M_{i-1}, 2|N_{i-1}|)$.
Hence, $P(i)$ holds.

\textbf{Case 3}: $k_i = 3$:
\\ Then $S_i = \ordSt(M_{i-1}, \{2|N_{i-1}|-1, 2|N_{i-1}|, 2|N_{i-1}|+1\})$,
$\ordSt(M_i, |N_i|) = \ordSt(M_{i-1}, |N_{i-1}|-1)$,
and $\ordSt(M_i, 2|N_i|) = \ordSt(M_{i-1}, 2|N_{i-1}|-2)$.
Hence, $P(i)$ holds.

\textbf{Case 4}: $k_i = 4$:
\\ Then $S_i = \ordSt(M_{i-1}, \{1, 2|N_{i-1}|+1\})$,
$\ordSt(M_i, 2|N_i|) = \ordSt(M_{i-1}, 2|N_{i-1}|-1)$,
and $\ordSt(M_i, |N_i|) = \ordSt(M_{i-1}, |N_{i-1}|)$.
Hence, $P(i)$ holds.

By mathematical induction, we get that $P(p)$ holds.
\end{proof}


==> prelims-extra.tex <==
\section{Missing Proofs of Section~\ref{sec:prelim}}
\label{sec:prelims-extra}

\loodVsTmms*
\begin{proof}
%All valuations considered in this proof are additive.

First, assume $1$-out-of-$d$ MMS allocations exist for all instances with $n$ agents. Consider any instance $\mathcal{I} = ([d], M, (v_1, \ldots, v_d))$ with $d$ agents. Then, for the instance $\mathcal{I}' = ([n], M, (v_1, \ldots, v_n))$, a $1$-out-of-$d$ MMS allocation $X'$ exists. Hence, $v_i(X_i') \ge \MMS_i^d(M)$ for all $i \in [n]$. Let $X$ be an allocation of $M$ over $d$ agents where $X_i = X_i'$ for $i \in [n]$ and $X_i = \emptyset$ for $i \in [d] \setminus [n]$. Then $X$ is a $T$-MMS allocation for $\mathcal{I}$. Since the choice of $\mathcal{I}$ was arbitrary, we get that $T$-MMS allocations exist for all instances with $d$ agents.

Now assume $T$-MMS allocations exist for all instances with $d$ agents.
Consider any instance $\mathcal{I} = ([n], M, (v_1, \ldots, v_n))$.
Add $d-n$ dummy agents with arbitrary additive valuations $v_{n+1}, \ldots, v_d$.
Let $\mathcal{I}' = ([d], M, (v_1, \ldots, v_d))$ be the resulting instance.
Then a $T$-MMS allocation $X'$ exists for $\mathcal{I}'$, i.e., $v_i(X_i') \ge \MMS_i^d(M)$ for all $i \in [n]$.
Hence, $X = (X_1', \ldots, X_n')$ is a 1-out-of-$d$ MMS allocation for $\mathcal{I}$.
Since the choice of $\mathcal{I}$ was arbitrary, we get that 1-out-of-$d$ MMS allocations exist for all instances with $n$ agents.
\end{proof}

\ordNorm*
\begin{proof}
    Let $\ins$ be an arbitrary instance. We create a $d$-normalized ordered instance $\mathcal{I}'' = (N, M, V'')$ such that from any $1$-out-of-$d$ MMS allocation for $\mathcal{I}''$, one can obtain a $1$-out-of-$d$ MMS allocation for the original instance $\mathcal{I}$.

    First of all, we can ignore all agents $i$ with $\MMS^d_i=0$ since no good needs to be allocated to them. Recall that for all $i \in N$, $P^i = (P^i_1, \ldots, P^i_d)$ is a $d$-MMS partition of agent $i$. For all $i \in N$ and $g \in M$, we define $v'_{i,g} = v_i(g)/v_i(P^i_j)$ where $j$ is such that $g \in P^i_j$. Now for all $i \in N$, let $v'_i: 2^M \rightarrow \mathbb{R}_{\geq 0}$ be defined as an additive function such that $v'_i(S)=\sum_{g \in S} v'_{i,g}$.  Note that $v'_{i,g} \leq v_i(g)/\MMS^d_i(M)$ for all $g \in M$ and thus,
    \begin{align}
        v_i(S) \geq v'_i(S) \cdot \MMS^d_i(M). \label{ineq-apx}
    \end{align}
    Since $v'_i(P^i_j)=1$ for all $i \in N$ and  $j \in [d]$, $\mathcal{I}' = (N, M, V')$ is a $d$-normalized instance. If a $1$-out-of-$d$ MMS allocation exists for $\mathcal{I}$, let $X$ be one such allocation. By Inequality \eqref{ineq-apx}, $v_i(X_i) \geq v'_i(X_i) \cdot \MMS^d_i(M) \geq \MMS^d_i(M)$. Thus, every allocation that is $1$-out-of-$d$ MMS for $\mathcal{I}'$ is $1$-out-of-$d$ MMS for $\mathcal{I}$ as well.
    For all agents $i$ and $g \in [m]$, let $v''_{i,g}$ be the $g$-th number in the multiset of $\{v_i(1), \ldots, v_i(m)\}$. Let $v''_i: 2^M \rightarrow \mathbb{R}_{\geq 0}$ be defined as an additive function such that $v''_i(S)=\sum_{g \in S} v''_{i,g}$. Let $\mathcal{I''} = (N,M,V'')$. Note that $\mathcal{I}''$ is ordered and $d$-normalized.
    Barman and Krishnamurthy \cite{barman2020approximation} proved that for any allocation $X$ in $\mathcal{I''}$, there exists and allocation $Y$ in $\mathcal{I'}$ such that $v'_i(Y_i) \geq v''_i(X_i)$. Therefore, from any $1$-out-of-$d$ MMS allocation in $\mathcal{I}''$, one can obtain a $1$-out-of-$d$ MMS allocation in $\mathcal{I'}$ and as already shown before, it gives a $1$-out-of-$d$ MMS allocation for $\mathcal{I}$.
\end{proof}

\begin{comment}
\validred*
\begin{proof} Clearly, $v_a(S) \geq 3/4$. Next, we show that the MMS values of all other agents do not decrease separately for each case of $S\in\{S_1,S_2, S_3,S_4\}$. Fix agent $b \in N \setminus \{a\}$ and a MMS partition $P^b=(P^b_1, \dots, P^b_n)$. After removing $S$, we show that a partition of $M \setminus S$ exists into $(n-1)$ bundles such that the value of each bundle is at least $1$.
\begin{itemize}
    \item \textbf{$S=S_1$. } Removal of one good from $P^b$ affects exactly one bundle and each of the remaining $(n-1)$ bundles has value at least $1$. Therefore, the MMS value of $b$ doesn't decrease.
    \item \textbf{$S=S_2$. } In $P^b$, there exists a bundle with two goods from $\{1, \dots, n+1\}$ (pigeonhole principle). Let $T$ be a bundle in $P^b$ that has two goods from $\{1, \dots,n+1\}$. Let us exchange these goods with goods $n$ and $n+1$ in other bundles and arbitrarily distribute any remaining goods in $T$ among other bundles. Clearly, the value of other bundles except $T$ does not decrease, and hence the MMS value of $b$ in the reduced instance doesn't decrease.
    \item \textbf{$S=S_3$. } Similar to the proof of Case $`S = S_2$'.
    \item \textbf{$S=S_4$.} In each iteration, the lowest index bundle from $\{S_1,S_2,S_3,S_4 \}$ is picked. Therefore, $S_4$ is only picked when $v_i(S_1),v_i(S_3) < 3/4$ for all $i \in N$ which implies that $v_{i1} < 3/4$ and $v_{i(2n+1)} < 1/4$ and hence $v_i(S_4) < 1$ for all $i\in N$.

    In $P^b$, if goods $1$ and $2n+1$ are in the same bundle, removing $S_4$ and agent $a$ is a valid reduction. For the other case, if $1$ and $2n+1$ are in two different bundles, we can make two new bundles, one with $\{1,2n+1\}$ and another with all the remaining goods of the two bundles. The value of the bundle without $\{1,2n+1\}$ is at least $1$ because $v_i(S_4) < 1$ for all $i\in N$ and $\MMS_i \ge 1$.
   Hence, this is a valid reduction. \qedhere
\end{itemize}
\end{proof}
\end{comment}


\propExact*
\begin{proof}
For the first part,
    fix an agent $i$. Let $1 \in P^i_1$. By Proposition \ref{prop:trivial}, $v_i(1) \leq v_i(P^i_1)=1$.

    For the second part, by the pigeonhole principle, there exists a bundle $P^i_k$ and two goods $j, j' \in \{1, 2, \ldots, d+1\}$ such that $\{j,j'\} \subseteq P^i_k$. Without loss of generality, assume $j < j'$. We have
    \begin{align*}
        v_i(C_d) &= v_i(d) + v_i(d+1) \tag{$C_d = \{d, d+1\}$}\\
        &\leq v_i(j) + v_i(j') &\tag{$j \leq d$ and $j' \leq d+1$} \\
        &\leq v_i(P^i_k) =1. &\tag{$\{j,j'\} \in P^i_k$}
    \end{align*}

    For the third part, we have
    \begin{align*}
        1 &\geq v_i(C_d) = v_i(d) + v_i(d+1) \geq 2 v_i(d+1).
    \end{align*}
    Thus, $v_i(d+1) \leq \tf12$.
\end{proof}

\lemCsum*
\begin{proof}
For the sake of contradiction, assume the claim does not hold for some agent $i$ and let $\ell \geq 1$ be the largest index for which we have $\sum_{j = \ell}^d v_i(C_j) > d - \ell + 1$. Proposition \ref{prop:exact}(\ref{exact:2}) implies that $\ell < d$.
We have
\begin{align*}
    v_i(\ell) + v_i(2d-\ell+1) &= v_i(C_\ell) \\
    &= \sum_{j=\ell}^d v_i(C_j) - \sum_{j=\ell+1}^d v_i(C_j) \\
    &>  (d - \ell + 1) - (d - (\ell+1) + 1) &\tag{$\sum_{j = k}^d v_i(C_j) \leq d - k + 1$ for $k>\ell$} \\
    &=1.
\end{align*}
 For all $j,j' < \ell$, $v_i(j) + v_i(j') \geq v_i(\ell) + v_i(2d-\ell+1) > 1$. Therefore, $j$ and $j'$ cannot be in the same bundle in any $d$-MMS partition of $i$. For $j<\ell$, let $j \in P^i_j$. For all $j<\ell$ and $\ell \leq j' \leq 2d-\ell+1$,
 \begin{align*}
    v_i(j) + v_i(j') &\geq v_i(\ell) + v_i(2d-\ell+1) \\
    &= v_i(C_{\ell}) >1.
 \end{align*}
 Therefore, $j' \notin P_j$. Also, since $\sum_{j = \ell}^d v_i(C_j) > d - \ell + 1$, there are at least $t \geq d-\ell+2$ different bundles $Q_1, \ldots, Q_t$ in $P$ such that $Q_j \cap \{\ell, \ldots, 2d-\ell+1\} \neq \emptyset$. It is a contradiction since these $t \geq d-\ell+2$ bundles must be different from $P^i_1, \ldots P^i_{\ell-1}$.
\end{proof}

